The Nature of Damped Lyman Alpha Systems and Their Hosts in the Standard Cold Dark Matter Universe

Using adaptive mesh-refinement cosmological hydrodynamic simulations with a physically motivated supernova feedback prescription we show that the standard cold dark matter model can account for extant observed properties of damped Lyman alpha systems (DLAs). We then examine the properties of DLA host galaxies. We find: (1) While DLA hosts roughly trace the overall population of galaxies at all redshifts, they are always gas rich. (2) The history of DLA evolution reflects primarily the evolution of the underlying cosmic density, galaxy size and galaxy interactions. With higher density and more interactions at high redshift DLAs are larger in both absolute terms and in relative terms with respect to virial radii of halos. (3) The variety of DLAs at high redshift is richer with a large contribution coming from galactic filaments, created through close galaxy interactions. The portion of gaseous disks of galaxies where most stars reside makes relatively small contribution to DLA incidence at z=3-4. (4) The vast majority of DLAs arise in halos of mass M_h=10^10-10^12 Msun at z=1.6-4. At z=3-4, 20-30% of DLA hosts are Lyman Break Galaxies (LBGs). (5) Galactic winds play an indispensable role in shaping the kinematic properties of DLAs. Specifically, the high velocity width DLAs are a mixture of those arising in high mass, high velocity dispersion halos and those arising in smaller mass systems where cold gas clouds are entrained to high velocities by galactic winds. (6) In agreement with observations, we see a weak but noticeable evolution in DLA metallicity. The metallicity distribution centers at [Z/H]=-1.5 to -1 at z=3-4, with the peak moving to [Z/H]=-0.75 at z=1.6 and [Z/H]=-0.5 by z=0. (7) The star formation rate of DLA hosts is concentrated in the range 0.3-30Msun/yr at z=3-4, gradually shifting lower to peak at ~0.5-1 Msun/yr by z=0.

==> addbib <==
@ARTICLE{2007Chung,
   author = {{Chung}, A. and {van Gorkom}, J.~H. and {Kenney}, J.~D.~P. and 
	{Vollmer}, B.},
    title = "{Virgo Galaxies with Long One-sided H I Tails}",
  journal = {\apjl},
   eprint = {arXiv:astro-ph/0703338},
 keywords = {Galaxies: Clusters: General, Galaxies: Evolution, Galaxies: Interactions, Galaxies: Kinematics and Dynamics},
     year = 2007,
    month = apr,
   volume = 659,
    pages = {L115-L119},
      doi = {10.1086/518034},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...659L.115C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1980Dressler,
   author = {{Dressler}, A.},
    title = "{Galaxy morphology in rich clusters - Implications for the formation and evolution of galaxies}",
  journal = {\apj},
 keywords = {ELLIPTICAL GALAXIES, GALACTIC CLUSTERS, GALACTIC EVOLUTION, GALACTIC STRUCTURE, SPIRAL GALAXIES, ASTRONOMICAL MAPS, DENSITY DISTRIBUTION, INTERSTELLAR GAS, TELESCOPES, UNIVERSE, X RAY ASTRONOMY},
     year = 1980,
    month = mar,
   volume = 236,
    pages = {351-365},
      doi = {10.1086/157753},
   adsurl = {http://adsabs.harvard.edu/abs/1980ApJ...236..351D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1997Dressler,
   author = {{Dressler}, A. and {Oemler}, Jr., A. and {Couch}, W.~J. and 
	{Smail}, I. and {Ellis}, R.~S. and {Barger}, A. and {Butcher}, H. and 
	{Poggianti}, B.~M. and {Sharples}, R.~M.},
    title = "{Evolution since Z = 0.5 of the Morphology-Density Relation for Clusters of Galaxies}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/9707232},
 keywords = {GALAXIES: CLUSTERS: GENERAL, GALAXIES: EVOLUTION, GALAXIES: STRUCTURE},
     year = 1997,
    month = dec,
   volume = 490,
    pages = {577-+},
      doi = {10.1086/304890},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...490..577D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2000Fasano,
   author = {{Fasano}, G. and {Poggianti}, B.~M. and {Couch}, W.~J. and {Bettoni}, D. and 
	{Kj{\ae}rgaard}, P. and {Moles}, M.},
    title = "{The Evolution of the Galactic Morphological Types in Clusters}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0005171},
 keywords = {Galaxies: Clusters: General, Galaxies: Evolution, Galaxies: Structure},
     year = 2000,
    month = oct,
   volume = 542,
    pages = {673-683},
      doi = {10.1086/317047},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...542..673F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2005Tran,
   author = {{Tran}, {K.-V.~H.} and {van Dokkum}, P. and {Illingworth}, G.~D. and 
	{Kelson}, D. and {Gonzalez}, A. and {Franx}, M.},
    title = "{Infall, the Butcher-Oemler Effect, and the Descendants of Blue Cluster Galaxies at z\~{}0.6}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0409696},
 keywords = {Galaxies: Clusters: Individual: Alphanumeric: MS 2053-04, Galaxies: Elliptical and Lenticular, cD, Galaxies: Evolution, Galaxies: Fundamental Parameters, Cosmology: Gravitational Lensing},
     year = 2005,
    month = jan,
   volume = 619,
    pages = {134-146},
      doi = {10.1086/426427},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...619..134T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2005Smith,
   author = {{Smith}, G.~P. and {Treu}, T. and {Ellis}, R.~S. and {Moran}, S.~M. and 
	{Dressler}, A.},
    title = "{Evolution since z = 1 of the Morphology-Density Relation for Galaxies}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0403455},
 keywords = {Galaxies: Clusters: General, Galaxies: Evolution, Galaxies: Formation, Galaxies: High-Redshift, Galaxies: Structure},
     year = 2005,
    month = feb,
   volume = 620,
    pages = {78-87},
      doi = {10.1086/426930},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...620...78S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2005Postman,
   author = {{Postman}, M. and {Franx}, M. and {Cross}, N.~J.~G. and {Holden}, B. and 
	{Ford}, H.~C. and {Illingworth}, G.~D. and {Goto}, T. and {Demarco}, R. and 
	{Rosati}, P. and {Blakeslee}, J.~P. and {Tran}, {K.-V.} and 
	{Ben{\'{\i}}tez}, N. and {Clampin}, M. and {Hartig}, G.~F. and 
	{Homeier}, N. and {Ardila}, D.~R. and {Bartko}, F. and {Bouwens}, R.~J. and 
	{Bradley}, L.~D. and {Broadhurst}, T.~J. and {Brown}, R.~A. and 
	{Burrows}, C.~J. and {Cheng}, E.~S. and {Feldman}, P.~D. and 
	{Golimowski}, D.~A. and {Gronwall}, C. and {Infante}, L. and 
	{Kimble}, R.~A. and {Krist}, J.~E. and {Lesser}, M.~P. and {Martel}, A.~R. and 
	{Mei}, S. and {Menanteau}, F. and {Meurer}, G.~R. and {Miley}, G.~K. and 
	{Motta}, V. and {Sirianni}, M. and {Sparks}, W.~B. and {Tran}, H.~D. and 
	{Tsvetanov}, Z.~I. and {White}, R.~L. and {Zheng}, W.},
    title = "{The Morphology-Density Relation in z \~{} 1 Clusters}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0501224},
 keywords = {Galaxies: Clusters: General, Galaxies: Evolution, Galaxies: Formation, Galaxies: Structure},
     year = 2005,
    month = apr,
   volume = 623,
    pages = {721-741},
      doi = {10.1086/428881},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...623..721P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{1999Poggianti,
   author = {{Poggianti}, B.~M. and {Smail}, I. and {Dressler}, A. and {Couch}, W.~J. and 
	{Barger}, A.~J. and {Butcher}, H. and {Ellis}, R.~S. and {Oemler}, Jr., A.
	},
    title = "{The Star Formation Histories of Galaxies in Distant Clusters}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/9901264},
 keywords = {GALAXIES: CLUSTERS: GENERAL, GALAXIES: EVOLUTION, GALAXIES: FUNDAMENTAL PARAMETERS, GALAXIES: STELLAR CONTENT},
     year = 1999,
    month = jun,
   volume = 518,
    pages = {576-593},
      doi = {10.1086/307322},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...518..576P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1984Haynes,
   author = {{Haynes}, M.~P. and {Giovanelli}, R. and {Chincarini}, G.~L.
	},
    title = "{The Influence of Envirionment on the H I Content of Galaxies}",
  journal = {\araa},
     year = 1984,
   volume = 22,
    pages = {445-470},
      doi = {10.1146/annurev.aa.22.090184.002305},
   adsurl = {http://adsabs.harvard.edu/abs/1984ARA%26A..22..445H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{1986Stark,
   author = {{Stark}, A.~A. and {Knapp}, G.~R. and {Bally}, J. and {Wilson}, R.~W. and 
	{Penzias}, A.~A. and {Rowe}, H.~E.},
    title = "{Molecules in galaxies. III - The Virgo cluster}",
  journal = {\apj},
 keywords = {INTERSTELLAR GAS, MOLECULAR GASES, VIRGO GALACTIC CLUSTER, CARBON MONOXIDE, DATA REDUCTION, EMISSIVITY, INFRARED SPECTRA, MASS DISTRIBUTION, MOLECULAR CLOUDS, RADIO SPECTRA},
     year = 1986,
    month = nov,
   volume = 310,
    pages = {660-678},
      doi = {10.1086/164717},
   adsurl = {http://adsabs.harvard.edu/abs/1986ApJ...310..660S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1989Kenney,
   author = {{Kenney}, J.~D.~P. and {Young}, J.~S.},
    title = "{The effects of environment on the molecular and atomic gas properties of large Virgo cluster spirals}",
  journal = {\apj},
 keywords = {GALACTIC EVOLUTION, MOLECULAR GASES, SPIRAL GALAXIES, VIRGO GALACTIC CLUSTER, ABUNDANCE, CARBON MONOXIDE, EMISSION SPECTRA, HYDROGEN, OPTICAL PROPERTIES, STAR FORMATION},
     year = 1989,
    month = sep,
   volume = 344,
    pages = {171-199},
      doi = {10.1086/167787},
   adsurl = {http://adsabs.harvard.edu/abs/1989ApJ...344..171K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{1990Cayatte,
   author = {{Cayatte}, V. and {van Gorkom}, J.~H. and {Balkowski}, C. and 
	{Kotanyi}, C.},
    title = "{VLA observations of neutral hydrogen in Virgo Cluster galaxies. I - The Atlas}",
  journal = {\aj},
 keywords = {H I REGIONS, HYDROGEN, INTERSTELLAR GAS, VERY LARGE ARRAY (VLA), VIRGO GALACTIC CLUSTER, RED SHIFT, SPIRAL GALAXIES, VELOCITY DISTRIBUTION},
     year = 1990,
    month = sep,
   volume = 100,
    pages = {604-634},
      doi = {10.1086/115545},
   adsurl = {http://adsabs.harvard.edu/abs/1990AJ....100..604C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003Treu,
   author = {{Treu}, T. and {Ellis}, R.~S. and {Kneib}, {J.-P.} and {Dressler}, A. and 
	{Smail}, I. and {Czoske}, O. and {Oemler}, A. and {Natarajan}, P.
	},
    title = "{A Wide-Field Hubble Space Telescope Study of the Cluster Cl 0024+16 at z = 0.4. I. Morphological Distributions to 5 Mpc Radius}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0303267},
 keywords = {Galaxies: Clusters: Individual: Alphanumeric: Cl 0024+1654, Galaxies: Evolution, Galaxies: Formation, Galaxies: Fundamental Parameters, Galaxies: High-Redshift, Galaxies: Photometry},
     year = 2003,
    month = jul,
   volume = 591,
    pages = {53-78},
      doi = {10.1086/375314},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...591...53T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{1988Warmels,
   author = {{Warmels}, R.~H.},
    title = "{The HI properties of spiral galaxies in the Virgo Cluster. III - The HI surface density distribution in 36 galaxies}",
  journal = {\aaps},
 keywords = {GALACTIC STRUCTURE, H I REGIONS, SPIRAL GALAXIES, VIRGO GALACTIC CLUSTER, CENTIMETER WAVES, DENSITY DISTRIBUTION, GALACTIC EVOLUTION},
     year = 1988,
    month = mar,
   volume = 72,
    pages = {427-447},
   adsurl = {http://adsabs.harvard.edu/abs/1988A%26AS...72..427W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2004Koopmann,
   author = {{Koopmann}, R.~A. and {Kenney}, J.~D.~P.},
    title = "{H{$\alpha$} Morphologies and Environmental Effects in Virgo Cluster Spiral Galaxies}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0406243},
 keywords = {Galaxies: Clusters: General, Galaxies: Clusters: Individual: Name: Virgo, Galaxies: Fundamental Parameters, Galaxies: Peculiar, Galaxies: Spiral, Galaxies: Structure},
     year = 2004,
    month = oct,
   volume = 613,
    pages = {866-885},
      doi = {10.1086/423191},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...613..866K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2005Crowl,
   author = {{Crowl}, H.~H. and {Kenney}, J.~D.~P. and {van Gorkom}, J.~H. and 
	{Vollmer}, B.},
    title = "{Dense Cloud Ablation and Ram Pressure Stripping of the Virgo Spiral NGC 4402}",
  journal = {\aj},
   eprint = {arXiv:astro-ph/0503422},
 keywords = {Galaxies: Clusters: General, Galaxies: Clusters: Individual: Name: Virgo, Galaxies: Evolution, Galaxies: ISM, Galaxies: Peculiar},
     year = 2005,
    month = jul,
   volume = 130,
    pages = {65-72},
      doi = {10.1086/430526},
   adsurl = {http://adsabs.harvard.edu/abs/2005AJ....130...65C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2004Kenney,
   author = {{Kenney}, J.~D.~P. and {van Gorkom}, J.~H. and {Vollmer}, B.
	},
    title = "{VLA H I Observations of Gas Stripping in the Virgo Cluster Spiral NGC 4522}",
  journal = {\aj},
   eprint = {arXiv:astro-ph/0403103},
 keywords = {Galaxies: Clusters: General, Galaxies: Clusters: Individual: Name: Virgo, Galaxies: Evolution, Galaxies: Interactions, Galaxies: ISM, Galaxies: Peculiar, Galaxies: Structure},
     year = 2004,
    month = jun,
   volume = 127,
    pages = {3361-3374},
      doi = {10.1086/420805},
   adsurl = {http://adsabs.harvard.edu/abs/2004AJ....127.3361K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2003Vollmer,
   author = {{Vollmer}, B.},
    title = "{NGC 4654: Gravitational interaction or ram pressure stripping?}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0211321},
 keywords = {galaxies: individual: NGC 4654, galaxies: interactions, galaxies: ISM, galaxies: kinematics and dynamics},
     year = 2003,
    month = feb,
   volume = 398,
    pages = {525-539},
      doi = {10.1051/0004-6361:20021729},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...398..525V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2005Vollmer,
   author = {{Vollmer}, B. and {Huchtmeier}, W. and {van Driel}, W.},
    title = "{NGC 4254: a spiral galaxy entering the Virgo cluster}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0505021},
 keywords = {galaxies: individual: NGC 4254, galaxies: interactions, galaxies: ISM, galaxies: kinematics and dynamics},
     year = 2005,
    month = sep,
   volume = 439,
    pages = {921-933},
      doi = {10.1051/0004-6361:20041350},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...439..921V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2005Oosterloo,
   author = {{Oosterloo}, T. and {van Gorkom}, J.},
    title = "{A large H I cloud near the centre of the Virgo cluster}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0505397},
 keywords = {intergalactic medium, galaxies: interaction, galaxies: clusters: individual: Virgo cluster, galaxies: individual: NGC 4388},
     year = 2005,
    month = jul,
   volume = 437,
    pages = {L19-L22},
      doi = {10.1051/0004-6361:200500127},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...437L..19O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



